Gene and RNA Editing: Methods, Enabling Technologies, Applications, and Future Directions

Gene and RNA editing methods, technologies, and applications are emerging as innovative forms of therapy and medicine, offering more efficient implementation compared to traditional pharmaceutical treatments. Current trends emphasize the urgent need for advanced methods and technologies to detect public health threats, including diseases and viral agents. Gene and RNA editing techniques enhance the ability to identify, modify, and ameliorate the effects of genetic diseases, disorders, and disabilities. Viral detection and identification methods present numerous opportunities for enabling technologies, such as CRISPR, applicable to both RNA and gene editing through the use of specific Cas proteins. This article explores the distinctions and benefits of RNA and gene editing processes, emphasizing their contributions to the future of medical treatment. CRISPR technology, particularly its adaptation via the Cas13 protein for RNA editing, is a significant advancement in gene editing. The article will delve into RNA and gene editing methodologies, focusing on techniques that alter and modify genetic coding. A-to-I and C-to-U editing are currently the most predominant methods of RNA modification. CRISPR stands out as the most cost-effective and customizable technology for both RNA and gene editing. Unlike permanent changes induced by cutting an individual's DNA genetic code, RNA editing offers temporary modifications by altering nucleoside bases in RNA strands, which can then attach to DNA strands as temporary modifiers.

==> comments_MR.tex <==
Related Works:

@article{gaj2021next,
  title={Next-generation CRISPR technologies and their applications in gene and cell therapy},
  author={Gaj, Thomas and others},
  journal={Trends in biotechnology},
  volume={39},
  number={7},
  pages={692--705},
  year={2021},
  publisher={Elsevier}
}

@article{bharathkumar2022crispr,
  title={CRISPR/Cas-based modifications for therapeutic applications: a review},
  author={Bharathkumar, Nagaraj and Sunil, Abraham and Meera, Prabhakar and Aksah, Sam and Kannan, Muthu and Saravanan, Konda Mani and Anand, Thirunavukarasou},
  journal={Molecular biotechnology},
  volume={64},
  number={4},
  pages={355--372},
  year={2022},
  publisher={Springer}
}

@article{liu2022crispr,
  title={The CRISPR-Cas toolbox and gene editing technologies},
  author={Liu, Guanwen and Lin, Qiupeng and Jin, Shuai and Gao, Caixia},
  journal={Molecular cell},
  volume={82},
  number={2},
  pages={333--347},
  year={2022},
  publisher={Elsevier}
}

@article{wang2023crispr,
  title={CRISPR technology: A decade of genome editing is only the beginning},
  author={Wang, Joy Y and Doudna, Jennifer A},
  journal={Science},
  volume={379},
  number={6629},
  pages={eadd8643},
  year={2023},
  publisher={American Association for the Advancement of Science}
}

@article{saber2023review,
  title={A review on advanced CRISPR-based genome-editing tools: base editing and prime editing},
  author={Saber Sichani, Ali and Ranjbar, Maryam and Baneshi, Maryam and Torabi Zadeh, Farid and Fallahi, Jafar},
  journal={Molecular Biotechnology},
  volume={65},
  number={6},
  pages={849--860},
  year={2023},
  publisher={Springer}
}

@article{villiger2024crispr,
  title={CRISPR technologies for genome, epigenome and transcriptome editing},
  author={Villiger, Lukas and Joung, Julia and Koblan, Luke and Weissman, Jonathan and Abudayyeh, Omar O and Gootenberg, Jonathan S},
  journal={Nature Reviews Molecular Cell Biology},
  pages={1--24},
  year={2024},
  publisher={Nature Publishing Group UK London}
}

@article{deneault2024recent,
  title={Recent Therapeutic Gene Editing Applications to Genetic Disorders},
  author={Deneault, Eric},
  journal={Current Issues in Molecular Biology},
  volume={46},
  number={5},
  pages={4147--4185},
  year={2024},
  publisher={MDPI}
}

@article{chehelgerdi2024comprehensive,
  title={Comprehensive review of CRISPR-based gene editing: mechanisms, challenges, and applications in cancer therapy},
  author={Chehelgerdi, Mohammad and Chehelgerdi, Matin and Khorramian-Ghahfarokhi, Milad and Shafieizadeh, Marjan and Mahmoudi, Esmaeil and Eskandari, Fatemeh and Rashidi, Mohsen and Arshi, Asghar and Mokhtari-Farsani, Abbas},
  journal={Molecular cancer},
  volume={23},
  number={1},
  pages={9},
  year={2024},
  publisher={Springer}
}
